Neutral meson production in d+Au and p+p collisions at sqrt(s_NN) = 200 GeV in STAR

The high centre-of-mass energy of 200 GeV available at the Relativistic Heavy Ion Collider (RHIC) at Brookhaven opens up the hard scattering regime in heavy-ion collisions. Particles at large transverse momentum originate from the early stage of the interaction and, therefore, probe the medium produced in these collisions. To quantitatively understand the medium induced modification of hadron production, precise measurements of identified hadrons in p+p and d+Au systems are required. This thesis presents the high transverse momentum measurements of neutral pions and eta mesons through their di-photon decay channel, performed with STAR Barrel Electromagnetic Calorimeter. The medium induced spectrum modification in d+Au collisions is also measured in comparison to the most peripheral d+Au and to the p+p collisions. The results are consistent with the previous STAR charged hadron measurements and with the theory (QCD) calculations, as well as with measurements from PHENIX, another RHIC experiment.

==> Makefile <==

LATEX = latex

BIBTEX = bibtex

DVIPS = dvips
DVIPS_OPTIONS = -Ppdf -z

PS2PDF = ps2pdf
PS2PDF_OPTIONS = -dOptimize=true -dEmbedAllFonts=true -dUseFlateCompression=true -dPDFSETTINGS=/prepress

LATEX2HTML = latex2html
LATEX2HTML_OPTIONS = -no_math -html_version 2.0,math -scalable_fonts

OUTPUT_DIR = ./output

.SUFFIXES: .tex .aux .toc .bbl .dvi .ps .pdf

.PHONY: all thesis title_page summary additional_summary electronics html \
    thesis_clean title_page_clean summary_clean additional_summary_clean electronics_clean \
    thesis_distclean title_page_distclean summary_distclean additional_summary_distclean electronics_distclean

all: thesis
#title_page 
#summary 
#additional_summary 
#electronics 
#html

clean: thesis_clean title_page_clean summary_clean additional_summary_clean electronics_clean html_clean

distclean: clean thesis_distclean title_page_distclean summary_distclean additional_summary_distclean electronics_distclean html_distclean

##################################################

thesis: ogrebeny_thesis.pdf

ogrebeny_thesis.pdf: ogrebeny_thesis.ps

ogrebeny_thesis.ps: ogrebeny_thesis.dvi

ogrebeny_thesis.dvi: ogrebeny_thesis.tex ogrebeny_thesis.aux ogrebeny_thesis.toc ogrebeny_thesis.bbl

ogrebeny_thesis.aux: ogrebeny_thesis.tex

ogrebeny_thesis.toc: ogrebeny_thesis.tex

ogrebeny_thesis.bbl: ogrebeny_thesis.aux

ogrebeny_thesis.aux ogrebeny_thesis.toc ogrebeny_thesis.dvi : \
    ogrebeny_commands.tex \
    title_page_cover.tex \
    title_page.tex \
    financing.tex \
    ogrebeny_EMC_electronics.tex \

thesis_clean:
	-rm ogrebeny_thesis.toc
	-rm ogrebeny_thesis.aux
	-rm ogrebeny_thesis.blg
	-rm ogrebeny_thesis.out
	-rm ogrebeny_thesis.log
	-rm ogrebeny_thesis.dvi
	-rm ogrebeny_thesis.ps
	-rm head.tmp
	-rm body.tmp

thesis_distclean:
	-rm ogrebeny_thesis.bbl
	-rm ogrebeny_thesis.pdf

##################################################

html:
	$(LATEX2HTML) $(LATEX2HTML_OPTIONS) ogrebeny_thesis.tex

html_clean:

html_distclean:
	-rm -fr ogrebeny_thesis

##################################################

title_page: ogrebeny_thesis_title_page.pdf

ogrebeny_thesis_title_page.pdf: ogrebeny_thesis_title_page.ps

ogrebeny_thesis_title_page.ps: ogrebeny_thesis_title_page.dvi

ogrebeny_thesis_title_page.dvi: ogrebeny_thesis_title_page.tex ogrebeny_thesis_title_page.aux

ogrebeny_thesis_title_page.aux: ogrebeny_thesis_title_page.tex

ogrebeny_thesis_title_page.aux ogrebeny_thesis_title_page.dvi: \
    ogrebeny_commands.tex \
    title_page.tex \
    financing.tex

title_page_clean:
	-rm ogrebeny_thesis_title_page.toc
	-rm ogrebeny_thesis_title_page.aux
	-rm ogrebeny_thesis_title_page.log
	-rm ogrebeny_thesis_title_page.dvi
	-rm ogrebeny_thesis_title_page.ps

title_page_distclean:
	-rm ogrebeny_thesis_title_page.pdf

##################################################

summary: ogrebeny_thesis_summary.pdf

ogrebeny_thesis_summary.pdf: ogrebeny_thesis_summary.ps

ogrebeny_thesis_summary.ps: ogrebeny_thesis_summary.dvi

ogrebeny_thesis_summary.dvi: ogrebeny_thesis_summary.tex ogrebeny_thesis_summary.aux

ogrebeny_thesis_summary.aux: ogrebeny_thesis_summary.tex

ogrebeny_thesis_summary.aux ogrebeny_thesis_summary.dvi: \
    ogrebeny_commands.tex \
    title_page.tex \
    financing.tex \
    summary.tex \
    samenvatting.tex

summary_clean:
	-rm ogrebeny_thesis_summary.toc
	-rm ogrebeny_thesis_summary.aux
	-rm ogrebeny_thesis_summary.log
	-rm ogrebeny_thesis_summary.dvi
	-rm ogrebeny_thesis_summary.ps

summary_distclean:
	-rm ogrebeny_thesis_summary.pdf

##################################################

additional_summary: ogrebeny_thesis_additional_summary.pdf

ogrebeny_thesis_additional_summary.pdf: ogrebeny_thesis_additional_summary.ps

ogrebeny_thesis_additional_summary.ps: ogrebeny_thesis_additional_summary.dvi

ogrebeny_thesis_additional_summary.dvi: ogrebeny_thesis_additional_summary.tex ogrebeny_thesis_additional_summary.aux

ogrebeny_thesis_additional_summary.aux: ogrebeny_thesis_additional_summary.tex

ogrebeny_thesis_additional_summary.aux ogrebeny_thesis_additional_summary.dvi: \
    ogrebeny_commands.tex \
    abstract.tex \
    keywords.tex \
    subject.tex \
    conclusions.tex \
    simple_summary.tex \
    simple_samenvatting.tex \
    financing.tex

additional_summary_clean:
	-rm ogrebeny_thesis_additional_summary.toc
	-rm ogrebeny_thesis_additional_summary.aux
	-rm ogrebeny_thesis_additional_summary.log
	-rm ogrebeny_thesis_additional_summary.dvi
	-rm ogrebeny_thesis_additional_summary.ps

additional_summary_distclean:
	-rm ogrebeny_thesis_additional_summary.pdf

##################################################

electronics: STAR_BEMC_electronics.pdf

STAR_BEMC_electronics.pdf: STAR_BEMC_electronics.ps

STAR_BEMC_electronics.ps: STAR_BEMC_electronics.dvi

STAR_BEMC_electronics.dvi: STAR_BEMC_electronics.tex STAR_BEMC_electronics.aux

STAR_BEMC_electronics.aux: STAR_BEMC_electronics.tex

STAR_BEMC_electronics.aux STAR_BEMC_electronics.dvi: \
    ogrebeny_commands.tex \
    ogrebeny_EMC_electronics.tex

electronics_clean:
	-rm STAR_BEMC_electronics.toc
	-rm STAR_BEMC_electronics.aux
	-rm STAR_BEMC_electronics.log
	-rm STAR_BEMC_electronics.dvi
	-rm STAR_BEMC_electronics.ps

electronics_distclean:
	-rm STAR_BEMC_electronics.pdf

##################################################

.tex.dvi:
	$(LATEX) $*
	$(LATEX) $*
	$(LATEX) $*

.tex.aux:
	$(LATEX) $*

.tex.toc:
	$(LATEX) $*

.aux.bbl:
	$(BIBTEX) $*

.dvi.ps:
	$(DVIPS) $(DVIPS_OPTIONS) $< -o $@

.ps.pdf:
	$(PS2PDF) $(PS2PDF_OPTIONS) $< $@


==> abstract.tex <==
The high centre-of-mass energy of 200 GeV available at the
Relativistic Heavy Ion Collider (RHIC) at Brookhaven opens up the hard
scattering regime in heavy-ion collisions. Particles at large transverse momentum originate
from the early stage of the interaction and, therefore, probe the medium
produced in these collisions.

To quantitatively understand the medium induced modification of hadron production, precise
measurements of identified hadrons in p+p and d+Au systems are required. 

This thesis presents the high transverse momentum measurements of neutral pions and eta mesons
through their di-photon decay channel, performed with STAR Barrel Electromagnetic Calorimeter.
The medium induced spectrum modification in d+Au collisions is also measured in comparison to 
the most peripheral d+Au and to the p+p collisions.

The results are consistent with the previous STAR charged hadron measurements and with the theory (QCD) calculations,
as well as with measurements from PHENIX, another RHIC experiment.


==> data_tables/table_eta_Rcp.tex <==
1.25    & 0.465    & 0.549     & 0.076     & 0.000     \\ 
1.75    & 1.057    & 0.539     & 0.191     & 0.000     \\ 
2.25    & 5.521    & 16.209     & 1.093     & 0.000     \\ 
2.75    & 0.176    & 1.016     & 0.038     & 0.000     \\ 
3.50    & 1.468    & 0.755     & 0.356     & 0.000     \\ 
4.50    & 3.358    & 3.082     & 0.936     & 0.142     \\ 
5.50    & 0.951    & 0.701     & 0.300     & 0.040     \\ 
6.50    & -0.198    & 4.077     & 0.000     & 0.000     \\ 
7.50    & 3.780    & 8.106     & 1.471     & 0.267     \\ 
9.00    & 0.100    & 7.923     & 0.044     & 0.007     \\ 
11.00\ \   & 0.559    & 1.770     & 0.291     & 0.040     \\ 
13.00\ \   & 0.471    & 2.078     & 0.280     & 0.033     \\ 
15.50\ \   & 0.853    & 1.788     & 0.587     & 0.060     \\ 

